Neutrinoless Double Beta Decay from Lattice QCD: The Long-Distance $\pi^{-} \rightarrow \pi^{+} e^{-} e^{-}$ Amplitude

Neutrinoless double beta decay (\( 0 \nu \beta \beta \)) is a hypothetical nuclear decay mode with important implications. In particular, observation of this decay would demonstrate that the neutrino is a Majorana particle and that lepton number conservation is violated in nature. Relating experimental constraints on \(0 \nu \beta \beta\) decay rates to the neutrino masses requires theoretical input in the form of non-perturbative nuclear matrix elements which remain difficult to calculate reliably. This work marks a first step toward providing a general lattice QCD framework for computing long-distance \(0 \nu \beta \beta\) matrix elements in the case where the decay is mediated by a light Majorana neutrino. The relevant formalism is developed and then tested by computing the simplest such matrix element describing an unphysical \( \pi^{-} \rightarrow \pi^{+} e^{-} e^{-} \) transition on a series of domain wall fermion ensembles. The resulting lattice data is then fit to next-to-leading-order chiral perturbation theory, allowing a fully-controlled extraction of the low energy constant governing the transition rate, \(g_{\nu}^{\pi \pi}(\mu = 770 \,\, \mathrm{MeV}) = -10.78(12)_{\rm stat}(51)_{\rm sys}\). Finally, future prospects for calculations of more complicated processes, such as the phenomenologically important \(n^{0} n^{0} \rightarrow p^{+} p^{+} e^{-} e^{-}\) decay, are discussed.

==> 4pt_int_sub.tex <==
This section presents Figure \ref{fig:lattice_4pt_data}, summarizing the data for the integrated four-point function defined by Eq.~\eqref{eqn:lattice_bilocal_me}. In Section \ref{subsec:LD_amplitude} the matrix element \(M^{0 \nu}\) \eqref{eqn:0vbb_me} is extracted by performing a series of linear fits to this data at large \(T\), including an estimate of the systematic uncertainty associated with the variation in \(M^{0 \nu}\) as the fit window is varied.

\begin{figure}[!ht]
\centering
\subfloat[24I ensembles]{\includegraphics[width=0.48\linewidth]{./figures/pion_0vbb_int_sub_24I_summary.pdf}}
\subfloat[32I ensembles]{\includegraphics[width=0.48\linewidth]{./figures/pion_0vbb_int_sub_32I_summary.pdf}}
\caption{Lattice signals for the integrated four-point function, Eq.~\eqref{eqn:lattice_bilocal_me}, after normalizing using Eq.~\eqref{eqn:normalized_4pt} and removing the exponentionally divergent contribution from the vacuum intermediate state using Eq.~\eqref{eqn:regulated_vacuum_4pt}.}
\label{fig:lattice_4pt_data}
\end{figure}

